Automatic Open-World Reliability Assessment

Image classification in the open-world must handle out-of-distribution (OOD) images. Systems should ideally reject OOD images, or they will map atop of known classes and reduce reliability. Using open-set classifiers that can reject OOD inputs can help. However, optimal accuracy of open-set classifiers depend on the frequency of OOD data. Thus, for either standard or open-set classifiers, it is important to be able to determine when the world changes and increasing OOD inputs will result in reduced system reliability. However, during operations, we cannot directly assess accuracy as there are no labels. Thus, the reliability assessment of these classifiers must be done by human operators, made more complex because networks are not 100% accurate, so some failures are to be expected. To automate this process, herein, we formalize the open-world recognition reliability problem and propose multiple automatic reliability assessment policies to address this new problem using only the distribution of reported scores/probability data. The distributional algorithms can be applied to both classic classifiers with SoftMax as well as the open-world Extreme Value Machine (EVM) to provide automated reliability assessment. We show that all of the new algorithms significantly outperform detection using the mean of SoftMax.

==> tbspace.tex <==
\makeatletter

\setlength\belowcaptionskip{6pt \@plus 4pt \@minus -6pt}
\setlength\abovecaptionskip{2pt}

% \long\def\@makecaption#1#2{
% \vspace*{\abovecaptionskip}
%    \setbox\@tempboxa\hbox{\small \noindent {\bf #1.}~{\it #2}}
%    \setlength{\@ctmp}{\hsize}
%    \addtolength{\@ctmp}{-\@figindent}\addtolength{\@ctmp}{-\@figindent}
%    % IF longer than one indented paragraph line
%    \ifdim \wd\@tempboxa >\@ctmp
%       % THEN DON'T set as an indented paragraph
%       {\small{\bf #1.}{~\it#2}\par}
%    \else
%       % ELSE center
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
%   \fi\vspace*{\belowcaptionskip}}

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-1.2ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-.6ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
	                           {\normalfont\large\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-.5ex\@plus -.2ex \@minus -.2ex}%
                                     {.2ex \@plus .2ex}%
                                     {\normalfont\large\bfseries}}

\abovedisplayskip=1pt plus 3pt minus 6pt 
\abovedisplayshortskip=0pt plus 3pt 
\belowdisplayskip=1pt plus 3pt minus 6pt 
\belowdisplayshortskip=0pt plus 3pt minus 3pt 

\floatsep 4pt plus 2pt minus 2pt 
\textfloatsep 4pt plus 2pt minus 4pt
\intextsep 2pt plus 2pt minus 2pt  
\dblfloatsep 4pt plus 2pt minus 2pt 
\dbltextfloatsep 6pt plus 2pt minus 4pt 
\@fptop 2pt plus 1fil \@fpsep 6pt plus 2fil \@fpbot 0pt plus 1fil 
\@dblfptop 6pt plus 1fil \@dblfpsep 6pt plus 2fil \@dblfpbot 2pt plus 1fil


\makeatother

\def\closemath{
\abovedisplayskip=3pt plus 3pt minus 1pt 
\abovedisplayshortskip=0pt plus 1pt minus 1pt 
\belowdisplayskip=3pt plus 3pt minus 1pt 
\belowdisplayshortskip=0pt plus 1pt minus 1pt }

\def\tightmath{
\abovedisplayskip=4pt plus 2pt minus 1pt 
\abovedisplayshortskip=2pt plus 1pt minus 1pt 
\belowdisplayskip=4pt plus 2pt minus 1pt 
\belowdisplayshortskip=2pt plus 1pt minus 1pt }
\def\crushmath{
\abovedisplayskip=1pt plus 1pt minus 2pt 
\abovedisplayshortskip=1pt plus 1pt minus 2pt 
\belowdisplayskip=1pt plus 1pt minus 2pt 
\belowdisplayshortskip=1pt plus 1pt minus 2pt }
\tightmath

